Understanding the Star Formation Efficiency in Dense Gas: Initial Results from the CAFFEINE Survey with ArT\'eMiS

Despite recent progress, the question of what regulates the star formation efficiency in galaxies remains one of the most debated problems in astrophysics. According to the dominant picture, star formation (SF) is regulated by turbulence and feedback, and the SFE is 1-2% per local free-fall time. In an alternate scenario, the SF rate in galactic disks is linearly proportional to the mass of dense gas above a critical density threshold. We aim to discriminate between these two pictures thanks to high-resolution observations tracing dense gas and young stellar objects (YSOs) for a comprehensive sample of 49 nearby massive SF complexes out to d < 3 kpc in the Galactic disk. We use data from CAFFEINE, a 350/450 $\mu$m survey with APEX/ArT\'eMiS of the densest portions of all southern molecular clouds, in combination with Herschel data to produce column density maps at 8" resolution. Our maps are free of saturation and resolve the structure of dense gas and the typical 0.1 pc width of molecular filaments at 3 kpc, which is impossible with Herschel data alone. Coupled with SFR estimates derived from Spitzer observations of the YSO content of the same clouds, this allows us to study the dependence of the SFE with density in the CAFFEINE clouds. We also combine our findings with existing SFE measurements in nearby clouds to extend our analysis down to lower column densities. Our results suggest that the SFE does not increase with density above the critical threshold and support a scenario in which the SFE in dense gas is approximately constant. However, the SFE measurements traced by Class I YSOs in nearby clouds are more inconclusive, since they are consistent with both the presence of a density threshold and a dependence on density above the threshold. Overall, we suggest that the SFE in dense gas is primarily governed by the physics of filament fragmentation into protostellar cores.

==> tex_table_CAFFEINE_SFR.tex <==
%\begin{sidewaystable*}
\longtab{
\begin{landscape}
\begin{longtable}{l|cccccc|cccccc}
\caption{\label{tab:CAFFEINE_sources_results} Derived properties for the CAFFEINE clouds}\\
%\begin{tabular}{lcccccccccccc}
\hline \hline
 & \multicolumn{6}{c|}{Clumps} & \multicolumn{6}{c}{YSOs}\\
Cloud & $N_{22.15}$\tablefootmark{a} & $N_{22.90}$\tablefootmark{a} & SFR$_{22.15}$\tablefootmark{b} & SFR$_{22.90}$\tablefootmark{b} & SFE$_{22.15}$ & SFE$_{22.90}$ & $N_{22.15}$\tablefootmark{c} & $N_{22.90}$\tablefootmark{c} & SFR$_{22.15}$\tablefootmark{d} & SFR$_{22.90}$\tablefootmark{d} & SFE$_{22.15}$ & SFE$_{22.90}$ \\
 &  &  & M$_\odot$\,Myr$^{-1}$ & M$_\odot$\,Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ &  &  & M$_\odot$\,Myr$^{-1}$ & M$_\odot$\,Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$\\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
 & \multicolumn{6}{c|}{Clumps} & \multicolumn{6}{c}{YSOs}\\
Cloud & $N_{22.15}$\tablefootmark{a} & $N_{22.90}$\tablefootmark{a} & SFR$_{22.15}$\tablefootmark{b} & SFR$_{22.90}$\tablefootmark{b} & SFE$_{22.15}$ & SFE$_{22.90}$ & $N_{22.15}$\tablefootmark{c} & $N_{22.90}$\tablefootmark{c} & SFR$_{22.15}$\tablefootmark{d} & SFR$_{22.90}$\tablefootmark{d} & SFE$_{22.15}$ & SFE$_{22.90}$ \\
 &  &  & M$_\odot$\,Myr$^{-1}$ & M$_\odot$\,Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ &  &  & M$_\odot$\,Myr$^{-1}$ & M$_\odot$\,Myr$^{-1}$ & $\times 10^{-8}$Myr$^{-1}$ & $\times 10^{-8}$yr$^{-1}$\\
\hline
\endhead
\hline
\multicolumn{13}{l}{
\tablefoot{
\tablefoottext{a}{Numbers of protostellar clumps identified within contours of $N_{\rm H_2}=10^{22.15}~\rm cm^{-2}$ and $N_{\rm H_2}=10^{22.90}~\rm cm^{-2}$, respectively.}
\tablefoottext{b}{Star formation rates within the same contours 
derived from protostellar clumps using the method described in Sect. \ref{sec:Meth_clump_relation}.}
\tablefoottext{c}{Numbers of Class~I and II YSOs identified within contours of $N_{\rm H_2}=10^{22.15}~\rm cm^{-2}$ and $N_{\rm H_2}=10^{22.90}~\rm cm^{-2}$, respectively.}
\tablefoottext{b}{Star formation rates within the same contours 
derived from YSOs using the method described in Sect.~\ref{sec:SFR-CAF-YSO}.}
}}
\endfoot
%%
MonR2 & 15 & 4 & 20 & 9 & 2.06 & 6.19 & 98 & 7 & 105 & 13 & 10.86 & 8.71 \\
R5180 & 6 & 3 & 159 & 98 & 2.45 & 2.3 & 5 & 0 & 106 & - & 1.64 & - \\
NGC2264 & 6 & 4 & 34 & 28 & 1.75 & 6.87 & 50 & 6 & 62 & 32 & 3.16 & 7.59 \\
GAL316 & 19 & 7 & 1152 & - & 10.71 & - & 30 & 5 & 84 & 89 & 0.78 & 3.06 \\
I14453 & 6 & 1 & 266 & - & 11.25 & - & 4 & 0 & - & - & - & - \\
SDC317p7 & 6 & 1 & 323 & - & 7.39 & - & 8 & 1 & 276 & - & 6.32 & - \\
SDC317p9 & 10 & 3 & 304 & - & 11.54 & - & 23 & 10 & 102 & 57 & 3.87 & 8.53 \\
RCW87 & 16 & 1 & 595 & - & 9.16 & - & 22 & 0 & 50 & - & 0.77 & - \\
G322 & 3 & 2 & - & - & - & - & 3 & 0 & - & - & - & - \\
SDC326 & 71 & 19 & 3700 & - & 6.5 & - & 91 & 18 & 574 & 190 & 1.01 & 1.16 \\
G327 & 11 & 3 & 446 & 179 & 2.23 & 1.82 & 14 & 2 & 187 & - & 0.94 & - \\
I15541 & 15 & 6 & 760 & 344 & 3.43 & 4.24 & 40 & 5 & 249 & 141 & 1.12 & 1.74 \\
GAL332 & 14 & 3 & 577 & 207 & 3.56 & 5.55 & 24 & 3 & 186 & - & 1.15 & - \\
G332 & 22 & 2 & 865 & - & 8.14 & - & 32 & 1 & 178 & - & 1.67 & - \\
RCW106 & 38 & 4 & 2136 & - & 3.35 & - & 64 & 2 & 456 & - & 0.72 & - \\
G333 & 5 & 1 & 236 & - & 7.38 & - & 6 & 0 & 266 & - & 8.33 & - \\
G333.2 & 36 & 10 & 3032 & 726 & 4.23 & 2.75 & 28 & 4 & 271 & - & 0.38 & - \\
I16175 & 4 & 1 & 148 & - & 2.51 & - & 6 & 2 & 273 & - & 4.6 & - \\
G337.1 & 6 & 0 & 54 & - & 5.09 & - & 18 & 0 & 338 & - & 31.91 & - \\
I16351 & 4 & 1 & 83 & 49 & 1.8 & 4.42 & 17 & 0 & 246 & - & 5.35 & - \\
I16367 & 6 & 1 & - & - & - & - & 21 & 5 & 233 & 72 & 7.14 & 17.36 \\
SDC338 & 30 & 9 & 930 & 414 & 4.42 & 9.76 & 62 & 9 & 922 & 142 & 4.38 & 3.34 \\
G337.9 & 11 & 1 & 683 & - & 5.88 & - & 22 & 2 & 356 & - & 3.07 & - \\
G339 & 8 & 2 & 286 & - & 9.95 & - & 24 & 4 & 251 & - & 8.71 & - \\
G340.8 & 6 & 2 & 284 & - & 3.2 & - & 13 & 2 & 103 & - & 1.17 & - \\
OH341 & 16 & 5 & 1144 & 398 & 7.04 & 9.68 & 33 & 7 & 256 & 178 & 1.57 & 4.34 \\
SDC340 & 15 & 7 & 370 & - & 7.1 & - & 40 & 9 & 76 & 105 & 1.46 & 7.74 \\
G341.9 & 2 & 2 & 370 & - & 4.24 & - & 4 & 0 & - & - & - & - \\
RCW116B & 14 & 5 & 550 & - & 9.07 & - & 26 & 5 & 291 & 290 & 4.81 & 17.59 \\
I16572 & 12 & 3 & 266 & - & 7.95 & - & 31 & 6 & 142 & 101 & 4.24 & 21.54 \\
SDC344 & 13 & 6 & 409 & 224 & 1.43 & 4.46 & 80 & 15 & 293 & 36 & 1.03 & 0.72 \\
SDC345.4 & 5 & 2 & 195 & - & 3.57 & - & 14 & 2 & 48 & - & 0.88 & - \\
SDC345.0 & 10 & 2 & 424 & - & 3.28 & - & 66 & 7 & 226 & 26 & 1.75 & 2.29 \\
SDC348 & 34 & 16 & 1891 & - & 9.75 & - & 54 & 20 & 141 & 179 & 0.73 & 2.66 \\
NGC6334N & 8 & 3 & 162 & - & 2.04 & - & 24 & 1 & 94 & - & 1.18 & - \\
I17233a & 4 & 3 & 61 & - & 8.93 & - & 12 & 7 & 99 & 161 & 14.48 & 61.92 \\
I17233b & 8 & 0 & 246 & - & 9.71 & - & 1 & 0 & - & - & - & - \\
NGC6357SE & 14 & 3 & 376 & - & 6.86 & - & 13 & 1 & 95 & - & 1.74 & - \\
OH353 & 10 & 5 & 1671 & - & 6.57 & - & 33 & 4 & 114 & - & 0.45 & - \\
G358.5 & 17 & 6 & 760 & - & 8.84 & - & 31 & 2 & 396 & - & 4.6 & - \\
G005 & 15 & 2 & - & - & - & - & 14 & 0 & 172 & - & 3.58 & - \\
G008 & 11 & 3 & 470 & - & 7.05 & - & 5 & 0 & 108 & - & 1.62 & - \\
SDC010 & 40 & 12 & 768 & 367 & 3.58 & 8.51 & 45 & 9 & 190 & 71 & 0.89 & 1.65 \\
G010 & 8 & 0 & 357 & - & 1.79 & - & 16 & 1 & 225 & - & 1.13 & - \\
W33 & 35 & 17 & 1671 & 905 & 1.07 & 2.84 & 142 & 18 & 513 & 258 & 0.33 & 0.81 \\
SDC014 & 22 & 4 & 708 & - & 4.82 & - & 82 & 13 & 237 & 83 & 1.61 & 3.97 \\
W42 & 5 & 0 & 267 & - & 2.58 & - & 5 & 1 & 1827 & - & 17.68 & - \\
G034 & 19 & 4 & 1193 & 474 & 1.24 & 3.34 & 65 & 5 & 645 & 476 & 0.67 & 3.35 \\
W48B & 11 & 4 & 323 & 240 & 2.8 & 6.21 & 40 & 5 & 314 & 262 & 2.72 & 6.79 \\
\hline
\end{longtable}
\end{landscape}
}

%\end{tabular}
%\end{sidewaystable*}

